Energy Efficiency in RIS-Aided Wireless Networks: Active or Passive RIS?

This work addresses the comparison between active and passive RISs in wireless networks, with reference to the system energy efficiency (EE). To provably convergent and computationally-friendly EE maximization algorithms are developed, which optimize the reflection coefficients of the RIS, the transmit powers, and the linear receive filters. Numerical results show the performance of the proposed methods and discuss the operating points in which active or passive RISs should be preferred from an energy-efficient perspective.

==> ICC 2023/abbreviations.tex <==
%\renewcommand{\arraystretch}{1.5}
%\newcommand{\spazio}{\rule[-6mm]{0mm}{0mm}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\wt}{\widetilde}
\newcommand{\ov}{\overline}
\newcommand{\LL}{{\cal L}}
\newcommand{\bN}{\mbox{\boldmath $N$}}
\newcommand{\br}{\mbox{\boldmath $r$}}
\newcommand{\bT}{\mbox{\boldmath $T$}}
\newcommand{\bJ}{\mbox{\boldmath $J$}}
\newcommand{\bs}{\mbox{\boldmath $s$}}
\newcommand{\uH}{\underline{H}}
\newcommand{\uh}{\underline{h}}
\newcommand{\bb}{\mbox{\boldmath $b$}}
\newcommand{\bbf}{\mbox{\boldmath $f$}}
\newcommand{\ba}{\mbox{\boldmath $a$}}
\newcommand{\bq}{\mbox{\boldmath $q$}}
\newcommand{\bp}{\mbox{\boldmath $p$}}
\newcommand{\be}{\mbox{\boldmath $e$}}
\newcommand{\bzero}{\mbox{\boldmath $0$}}
\newcommand{\bM}{\mbox{\boldmath $M$}}
\newcommand{\wi}{\widetilde}
\newcommand{\bDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\wh}{\widehat}
\newcommand{\bA}{\mbox{\boldmath $A$}}
\newcommand{\bP}{\mbox{\boldmath $P$}}
\newcommand{\bC}{\mbox{\boldmath $C$}}
\newcommand{\bX}{\mbox{\boldmath $X$}}
\newcommand{\bh}{\mbox{\boldmath $h$}}
\newcommand{\bH}{\mbox{\boldmath $H$}}
\newcommand{\bK}{\mbox{\boldmath $K$}}
\newcommand{\bk}{\mbox{\boldmath $k$}}
\newcommand{\bc}{\mbox{\boldmath $c$}}
\newcommand{\bS}{\mbox{\boldmath $S$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bZ}{\mbox{\boldmath $Z$}}
\newcommand{\bU}{\mbox{\boldmath $U$}}
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bB}{\mbox{\boldmath $B$}}
\newcommand{\bE}{\mbox{\boldmath $E$}}
\newcommand{\bV}{\mbox{\boldmath $V$}}
\newcommand{\bL}{\mbox{\boldmath $L$}}
\newcommand{\bG}{\mbox{\boldmath $G$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bW}{\mbox{\boldmath $W$}}
\newcommand{\bLambda}{{\bf \Lambda}}
\newcommand{\bpsi}{{\bf \Psi}}
\newcommand{\bPsi}{{\bf \Psi}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
%\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bi}{\mbox{\boldmath $i$}}
\newcommand{\bu}{\mbox{\boldmath $u$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\bdelta}{\mbox{\boldmath $\delta$}}
\newcommand{\bx}{\mbox{\boldmath $x$}}
\newcommand{\bz}{\mbox{\boldmath $z$}}
\newcommand{\bg}{\mbox{\boldmath $g$}}
\newcommand{\bn}{\mbox{\boldmath $n$}}
\newcommand{\bbm}{\mbox{\boldmath $m$}}
\newcommand{\bv}{\mbox{\boldmath $v$}}
\newcommand{\bd}{\mbox{\boldmath $d$}}
\newcommand{\bQ}{\mbox{\boldmath $Q$}}
\newcommand{\bO}{\mbox{\boldmath $O$}}
\newcommand{\bR}{\mbox{\boldmath $R$}}
\newcommand{\bF}{\mbox{\boldmath $F$}}
\newcommand{\bphi}{{\bf \Phi}}
\newcommand{\bI}{\mbox{\boldmath $I$}}
\newcommand{\bbtheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\bSigma}{{\bf \Sigma}}
\newcommand{\bt}{\mbox{\boldmath $t$}}
\newcommand{\bD}{\mbox{\boldmath $D$}}
\newcommand{\by}{\mbox{\boldmath $y$}}
\newcommand{\ds}{\displaystyle}
\newcommand{\bw}{\mbox{\boldmath $w$}}
\newcommand{\bY}{\mbox{\boldmath $Y$}}
\newcommand{\K}{{\cal K}}
\newcommand{\G}{{\cal G}}
\newcommand{\N}{{\cal N}_0}
\hyphenation{E-let-tro-ni-ca}
\newcommand{\bbeta}{\mbox{\boldmath{$\beta$}}}
\def\M{{\cal M}}
\def\R{{\cal R}}
\def\S{{\cal S}}
\def\I{{\cal I}}
\newcommand{\beq}{\begin{equation}}

% Set of real, integer, etc., numbers, l_2 spaces, real, and imaginary parts
\newcommand{\Reals}    {{\mathbb R}} % {{{\mathrm I\!R}}}  
\newcommand{\Cplx}      {{{\mathsf I}\!\!\!{\mathrm C}}} %{{\mathbb C}}
\newcommand{\NCplx}     {{{\mathcal{CN}}}} % Complex normal distribution
\newcommand{\Ints}      {{{\mathbb Z}}} % Z set of all integers
\newcommand{\Rats}      {{{\mathsf I}\!\!\!{\mathrm Q}}}    % Q set of all rational numbers
\newcommand{\Nats}      {{{\mathrm{ I\!N}}}} % N set of all natural numbers
\newcommand{\Tee}{      {{\mathbb T}}}
\newcommand{\ltwo}      {{\ell_2}}
\newcommand{\lone}      {{\ell_1}}
\newcommand{\Ltwo}      {{\mathbb L}^2}
\newcommand{\LtR}       {\Ltwo(\Reals)}
\newcommand{\Real}[1]   {{\mathrm{Re}\left\{#1\right\}}}
\newcommand{\Imag}[1]   {{\mathrm{Im}\left\{#1\right\}}}
\newcommand{\real}      {{\mathcal{R}} e}
\newcommand{\imag}      {{\mathcal{I}} m}



% Some commands for nice typesetting
\newcommand{\ie}        {i.~e., \hspace{2pt}}      % id est
\newcommand{\eg}        {e.~g., \hspace{2pt}}      %
\newcommand{\define}    {\stackrel{\triangle}{=}}  % define, an '=' with an '^' on top
\newcommand{\D}  {^{\dag}}               % Dagger, includes '^' !
\newcommand{\T}  {{\mathsf{T}}}          % Transpose, no '^' !
\newcommand{\ct} {{\mathsf{*}}}          % conjugate complex, should use \dag for conjugate complex transpose
\newcommand{\half}{{{^1\!\!\scriptscriptstyle{/}\!}_2}}       % a nice 1/2
\newcommand{\mrsss}[1]   {{\mathrm{\scriptscriptstyle{#1}}}}  % math roman scriptscriptstyle - works well for sub and superscripts
\newcommand{\sth}     {{\mathrm{th}}}    % superscript th \th is already defined -- the $k^\sth$ user
\newcommand{\diag}    {{\mathrm{diag}}}  % for diag{1, 2, 3}
\newcommand{\tr}      {{\mathrm{tr}}}    % trace of a matrix
\newcommand{\Res}     {{\mathrm{Res}}}   % Residue
\newcommand{\ld}      {{\mathrm{ld}}}    % logarithmus dualis
\newcommand{\barg}    {\overline{\gamma}}     % average received SNR
\newcommand{\sqgb}    {\sqrt{\barg}}     % square root of the average received SNR
\newcommand{\e}       {{\mathrm e}}      % e for exponential function
\newcommand{\E}       {{\mathrm E}}      % Expectation
\newcommand{\lNZ}     {{\lambda_{\mathsf{NZ}}}} % to denote the non-zero eigenvalues of a matrix
\newcommand{\Mt}      {{M_{\!\mrsss{T}}}}% N_T no of transmit antennas
\newcommand{\Mr}      {{M_{\!\mrsss{R}}}}% N_R no of receive antennas
\newcommand{\uple}    {{\mathrm{ul}}}    % upper-left
\newcommand{\upri}    {{\mathrm{ur}}}    % upper-right
\newcommand{\lole}    {{\mathrm{ll}}}    % lower-left
\newcommand{\lori}    {{\mathrm{lr}}}    % lower-right

% Bold numbers
\newcommand{\Zrb}     {{\mathbf 0}}      % bold zero
\newcommand{\Oneb}    {{\mathbf 1}}      % bold one

% Define bold roman letters
\newcommand{\ab}{{\mathbf a}}  \newcommand{\Ab}{{\mathbf A}}
\newcommand{\cb}{{\mathbf c}}  \newcommand{\Cb}{{\mathbf C}}
\newcommand{\db}{{\mathbf d}}  \newcommand{\Db}{{\mathbf D}}
\newcommand{\eb}{{\mathbf e}}  \newcommand{\Eb}{{\mathbf E}}
\newcommand{\fb}{{\mathbf f}}  \newcommand{\Fb}{{\mathbf F}}
\newcommand{\gb}{{\mathbf g}}  \newcommand{\Gb}{{\mathbf G}}
\newcommand{\hb}{{\mathbf h}}  \newcommand{\Hb}{{\mathbf H}}
\newcommand{\ib}{{\mathbf i}}  \newcommand{\Ib}{{\mathbf I}}
\newcommand{\jb}{{\mathbf j}}  \newcommand{\Jb}{{\mathbf J}}
\newcommand{\kb}{{\mathbf k}}  \newcommand{\Kb}{{\mathbf K}}
\newcommand{\lb}{{\mathbf l}}  \newcommand{\Lb}{{\mathbf L}}
\newcommand{\mb}{{\mathbf m}}  \newcommand{\Mb}{{\mathbf M}}
\newcommand{\nb}{{\mathbf n}}  \newcommand{\Nb}{{\mathbf N}}
\newcommand{\ob}{{\mathbf o}}  \newcommand{\Ob}{{\mathbf O}}
\newcommand{\pb}{{\mathbf p}}  \newcommand{\Pb}{{\mathbf P}}
\newcommand{\qb}{{\mathbf q}}  \newcommand{\Qb}{{\mathbf Q}}
\newcommand{\rb}{{\mathbf r}}  \newcommand{\Rb}{{\mathbf R}}
\renewcommand{\sb}{{\mathbf s}}\newcommand{\Sb}{{\mathbf S}} %\sb is equiv. to _ in Tex, unnecessary.
\newcommand{\tb}{{\mathbf t}}  \newcommand{\Tb}{{\mathbf T}}
\newcommand{\ub}{{\mathbf u}}  \newcommand{\Ub}{{\mathbf U}}
\newcommand{\vb}{{\mathbf v}}  \newcommand{\Vb}{{\mathbf V}}
\newcommand{\wb}{{\mathbf w}}  \newcommand{\Wb}{{\mathbf W}}
\newcommand{\xb}{{\mathbf x}}  \newcommand{\Xb}{{\mathbf X}}
\newcommand{\yb}{{\mathbf y}}  \newcommand{\Yb}{{\mathbf Y}}
\newcommand{\zb}{{\mathbf z}}  \newcommand{\Zb}{{\mathbf Z}}

% Define bold greek letters, lower and upper case
\newcommand{\alphab}      {{\bm \alpha}}          \newcommand{\Alphab}   {{\mathbf {\mathrm A}}}
\newcommand{\betab}       {{\bm \beta}}           \newcommand{\Betab}    {{\mathbf {\mathrm B}}}
\newcommand{\gammab}      {{\bm \gamma}}          \newcommand{\Gammab}   {{\bm \Gamma}}
\newcommand{\deltab}      {{\bm \delta}}          \newcommand{\Deltab}   {{\bm \Delta}}
\newcommand{\epsilonb}    {{\bm \epsilon}}        \newcommand{\Epsilonb} {{\mathbf {\mathrm E}}}
\newcommand{\varepsilonb} {{\bm \varepsilon}}
\newcommand{\vepsilonb}   {{\bm \varepsilon}}
\newcommand{\zetab}       {{\bm \zeta}}           \newcommand{\Zetab}    {{\mathbf {\mathrm Z}}}
\newcommand{\etab}        {{\bm \eta}}            \newcommand{\Etab}     {{\mathbf {\mathrm H}}}
\newcommand{\thetab}      {{\bm \theta}}          \newcommand{\Thetab}   {{\bm \Theta}}
\newcommand{\varthetab}   {{\bm \vartheta}}
\newcommand{\vthetab}     {{\bm \vartheta}}
\newcommand{\iotab}       {{\bm \iota}}           \newcommand{\Iotab}    {{\mathbf {\mathrm I}}}
\newcommand{\kappab}      {{\bm \kappa}}          \newcommand{\Kappab}   {{\mathbf {\mathrm K}}}
\newcommand{\lambdab}     {{\bm \lambda}}         \newcommand{\Lambdab}  {{\bm \Lambda}}
\newcommand{\mub}         {{\bm \mu}}             \newcommand{\Mub}      {{\mathbf {\mathrm M}}}
\newcommand{\nub}         {{\bm \nu}}             \newcommand{\Nub}     	{{\mathbf {\mathrm N}}}	
\newcommand{\xib}         {{\bm \xi}}             \newcommand{\Xib}      {{\bm \Xi}}
\newcommand{\omicronb}    {{\mathbf {\mathrm o}}} \newcommand{\Omicronb} {{\mathbf {\mathrm O}}}
\newcommand{\pib}         {{\bm \pi}}             \newcommand{\Pib}      {{\bm \Pi}}
\newcommand{\varpib}      {{\bm \varpi}}
\newcommand{\vpib}        {{\bm \varpi}}
\newcommand{\rhob}        {{\bm \rho}}            \newcommand{\Rhob}     {{\mathbf {\mathrm P}}}
\newcommand{\varrhob}     {{\bm \varrho}}
\newcommand{\vrhob}       {{\bm \varrho}}
\newcommand{\sigmab}      {{\bm \sigma}}          \newcommand{\Sigmab}   {{\bm \Sigma}}
\newcommand{\varsigmab}   {{\bm \varsigma}}
\newcommand{\vsigmab}     {{\bm \varsigma}}
\newcommand{\taub}        {{\bm \tau}}            \newcommand{\Taub}     {{\mathbf {\mathrm T}}}
\newcommand{\upsilonb}    {{\bm \upsilon}}        \newcommand{\Upsilonb} {{\bm \Upsilon}}
\newcommand{\phib}        {{\bm \phi}}            \newcommand{\Phib}     {{\bm \Phi}}
\newcommand{\varphib}     {{\bm \varphi}}
\newcommand{\vphib}       {{\bm \varphi}}
\newcommand{\chib}        {{\bm \chi}}            \newcommand{\Chib}     {{\mathbf {\mathrm X}}}
\newcommand{\psib}        {{\bm \psi}}            \newcommand{\Psib}     {{\bm \Psi}}
\newcommand{\omegab}      {{\bm \omega}}          \newcommand{\Omegab}   {{\bm \Omega}}

% Calligraphic letters, normal and bold
\newcommand{\Ac} {{\mathcal A}}         \newcommand{\Ak} {{\bm {\mathcal A}}}
\newcommand{\Bc} {{\mathcal B}}         \newcommand{\Bk} {{\bm {\mathcal B}}}
\newcommand{\Cc} {{\mathcal C}}         \newcommand{\Ck} {{\bm {\mathcal C}}}
\newcommand{\Dc} {{\mathcal D}}         \newcommand{\Dk} {{\bm {\mathcal D}}}
\newcommand{\Ec} {{\mathcal E}}         \newcommand{\Ek} {{\bm {\mathcal E}}}
\newcommand{\Fc} {{\mathcal F}}         \newcommand{\Fk} {{\bm {\mathcal F}}}
\newcommand{\Gc} {{\mathcal G}}         \newcommand{\Gk} {{\bm {\mathcal G}}}
\newcommand{\Hc} {{\mathcal H}}         \newcommand{\Hk} {{\bm {\mathcal H}}}
\newcommand{\Ic} {{\mathcal I}}         \newcommand{\Ik} {{\bm {\mathcal I}}}
\newcommand{\Jc} {{\mathcal J}}         \newcommand{\Jk} {{\bm {\mathcal J}}}
\newcommand{\Kc} {{\mathcal K}}         \newcommand{\Kk} {{\bm {\mathcal K}}}
\newcommand{\Lc} {{\mathcal L}}         \newcommand{\Lk} {{\bm {\mathcal L}}}
\newcommand{\Mc} {{\mathcal M}}         \newcommand{\Mk} {{\bm {\mathcal M}}}
\newcommand{\Nc} {{\mathcal N}}         \newcommand{\Nk} {{\bm {\mathcal N}}}
\newcommand{\Oc} {{\mathcal O}}         \newcommand{\Ok} {{\bm {\mathcal O}}}
\newcommand{\Pc} {{\mathcal P}}         \newcommand{\Pk} {{\bm {\mathcal P}}}
\newcommand{\Qc} {{\mathcal Q}}         \newcommand{\Qk} {{\bm {\mathcal Q}}}
\newcommand{\Rc} {{\mathcal R}}         \newcommand{\Rk} {{\bm {\mathcal R}}}
\newcommand{\Sc} {{\mathcal S}}         \newcommand{\Sk} {{\bm {\mathcal S}}}
\newcommand{\Tc} {{\mathcal T}}         \newcommand{\Tk} {{\bm {\mathcal T}}}
\newcommand{\Uc} {{\mathcal U}}         \newcommand{\Uk} {{\bm {\mathcal U}}}
\newcommand{\Vc} {{\mathcal V}}         \newcommand{\Vk} {{\bm {\mathcal V}}}
\newcommand{\Wc} {{\mathcal W}}         \newcommand{\Wk} {{\bm {\mathcal W}}}
\newcommand{\Xc} {{\mathcal X}}         \newcommand{\Xk} {{\bm {\mathcal X}}}
\newcommand{\Yc} {{\mathcal Y}}         \newcommand{\Yk} {{\bm {\mathcal Y}}}
\newcommand{\Zc} {{\mathcal Z}}         \newcommand{\Zk} {{\bm {\mathcal Z}}}


\newcommand{\Grb}   {{\mathbf {\mathrm V}}}

\newcommand{\Qulk} {{\underline{{\bm {\mathcal Q}}}}}

\newcommand{\Gulc} {{\underline{\mathcal G}}}
\newcommand{\Culc} {{\underline{\mathcal C}}}

% underlined upper and lower case letters
\newcommand{\Aul}  {{\underline A}}              \newcommand{\aul}  {{\underline a}}
\newcommand{\Bul}  {{\underline B}}              \newcommand{\bul}  {{\underline b}}
\newcommand{\Cul}  {{\underline C}}              \newcommand{\cul}  {{\underline c}}
\newcommand{\Dul}  {{\underline D}}              \newcommand{\dul}  {{\underline d}}
\newcommand{\Eul}  {{\underline E}}              \newcommand{\eul}  {{\underline e}}
\newcommand{\Ful}  {{\underline F}}              \newcommand{\ful}  {{\underline f}}
\newcommand{\Gul}  {{\underline G}}              \newcommand{\gul}  {{\underline g}}
\newcommand{\Hul}  {{\underline H}}              \newcommand{\hul}  {{\underline h}}
\newcommand{\Iul}  {{\underline I}}              \newcommand{\iul}  {{\underline i}}
\newcommand{\Jul}  {{\underline J}}              \newcommand{\jul}  {{\underline j}}
\newcommand{\Kul}  {{\underline K}}              \newcommand{\kul}  {{\underline k}}
\newcommand{\Lul}  {{\underline L}}              \newcommand{\lul}  {{\underline l}}
\newcommand{\Mul}  {{\underline M}}              \newcommand{\mull} {{\underline m}}
\newcommand{\Nul}  {{\underline N}}              \newcommand{\nul}  {{\underline n}}
\newcommand{\Oul}  {{\underline 0}}              \newcommand{\oul}  {{\underline o}}
\newcommand{\Pul}  {{\underline P}}              \newcommand{\pul}  {{\underline p}}
\newcommand{\Qul}  {{\underline Q}}              \newcommand{\qul}  {{\underline q}}
\newcommand{\Rul}  {{\underline R}}              \newcommand{\rul}  {{\underline r}}
\newcommand{\Sul}  {{\underline S}}              \newcommand{\sul}  {{\underline s}}
\newcommand{\Tul}  {{\underline T}}              \newcommand{\tul}  {{\underline t}}
\newcommand{\Uul}  {{\underline U}}              \newcommand{\uul}  {{\underline u}}
\newcommand{\Vul}  {{\underline V}}              \newcommand{\vul}  {{\underline v}}
\newcommand{\Wul}  {{\underline W}}              \newcommand{\wul}  {{\underline w}}
\newcommand{\Xul}  {{\underline X}}              \newcommand{\xul}  {{\underline x}}
\newcommand{\Yul}  {{\underline Y}}              \newcommand{\yul}  {{\underline y}}
\newcommand{\Zul}  {{\underline Z}}              \newcommand{\zul}  {{\underline z}}

% Misc. short-cuts
\newcommand{\mc}[1]     {{\mathcal{#1}}}        % mathcal
\newcommand{\what}[1]   {\widehat{#1}}          % widehat
\newcommand{\wtld}[1]   {\widetilde{#1}}        % widetilde
\newcommand{\Portho}[1] {\Pb_{#1}^{\perp}}      % orthogonal projection

%\newcounter{MYtempeqncnt}
%\setlength\arraycolsep{2pt} \sloppy

%\newcommand{\threshold}{\mbox{$
%\begin{array}{c} \stackrel{\textstyle H_1}{\textstyle>}\\
%\stackrel{\textstyle <}{\textstyle H_0}
%\end{array}$}}
%\newcommand{\nchoosek}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
%\newcommand{\gammabar}{\bar{\gamma}}
%\newcommand{\Prob}{\mbox{Prob}}

%\def\QED{\mbox{\rule[0pt]{1.5ex}{1.5ex}}}
%\setlength\arraycolsep{2pt} \sloppy

\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
%\newtheorem{algorithm}{Algorithm}
%\newtheorem{proof}{Proof}

\def\IR{{\mathbb R}}
\def\IC{{\mathbb C}}


==> ICC 2023/acronyms.tex <==
\makeglossaries

\newacronym{mac}{MAC}{multiple-access channel}
\newacronym{bc}{BC}{broadcast channel}
\newacronym{mimo}{MIMO}{multiple-input multiple-output}
\newacronym{siso}{SISO}{single-input single-output}
\newacronym{sc}{SC}{single-carrier}
\newacronym{mc}{MC}{multi-carrier}
\newacronym{ofdma}{OFDMA}{orthogonal frequency division multiple access}
\newacronym{af}{AF}{amplify-and-forward}
\newacronym{df}{DF}{decode-and-forward}
\newacronym{cf}{CF}{compress-and-forward}
\newacronym{mwrc}{MWRC}{multi-way relay channel}
\newacronym{pde}{PDE}{partial data exchange}
\newacronym{fde}{FDE}{full data exchange}
\newacronym{iid}{i.i.d.\@}{independent and identically distributed}
\newacronym{awgn}{AWGN}{additive white Gaussian noise}
\newacronym{awg}{AWG}{additive white Gaussian}
\newacronym{sic}{SIC}{successive interference cancellation}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{sinr}{SINR}{signal-to-interference-plus-noise ratio}
\newacronym{ber}{BER}{bit error rate}
\newacronym{zf}{ZF}{zero-forcing}
\newacronym{mmse}{MMSE}{minimum mean square error}
\newacronym{sud}{SUD}{single user decoding}
\newacronym{dof}{DoF}{degrees of freedom}
\newacronym{gdof}{GDoF}{generalized degrees of freedom}
\newacronym{nnc}{NNC}{noisy network coding}
\newacronym{dmn}{DMN}{discrete memoryless network}
\newacronym{csi}{CSI}{channel state information}
\newacronym{ee}{EE}{energy efficiency}
\newacronym{ian}{IAN}{treating interference as noise}
\newacronym{snd}{SND}{simultaneous non-unique decoding}
\newacronym{brd}{BRD}{best response dynamics}
\newacronym{br}{BR}{best response}
\newacronym{ne}{NE}{Nash equilibrium}
\newacronym{lhs}{LHS}{left-hand side}
\newacronym{rhs}{RHS}{right-hand side}
\newacronym{gee}{GEE}{global energy efficiency}
\newacronym{wsee}{WSEE}{weighted sum energy efficiency}
\newacronym{wpee}{WPEE}{weighted product energy efficiency}
\newacronym{wmee}{WMEE}{weighted minimum energy efficiency}
\newacronym{kkt}{KKT}{Karush-Kuhn-Tucker}
\newacronym{pc}{PC}{pseudo-concave}
\newacronym{qc}{QC}{quasi-concave}
\newacronym{ql}{QL}{quasi-linear}
\newacronym{pl}{PL}{pseudo-linear}
\newacronym{spc}{SPC}{strictly pseudo-concave}
\newacronym{sqc}{SQC}{strictly quasi-concave}
\newacronym{lfp}{LFP}{linear fractional problem}
\newacronym{clfp}{CLFP}{concave-linear fractional problem}
\newacronym{ccfp}{CCFP}{concave-convex fractional problem}
\newacronym{mmfp}{MMFP}{max-min fractional problem}
\newacronym{sorp}{SoRP}{sum-of-ratios problem}
\newacronym{porp}{PoRP}{product-of-ratios problem}
\newacronym{srp}{SRP}{single-ratio problem}
\newacronym{brb}{BRB}{branch-reduce-and-bound}
\newacronym{qos}{QoS}{quality-of-service}
\newacronym{comp}{CoMP}{cooperative multi-point}
\newacronym{ue}{UE}{user equipment}
\newacronym{bs}{BS}{base station}
\newacronym{mrc}{MRC}{maximum ratio combining}
\newacronym{d2d}{D2D}{device-to-device}
\newacronym{lmmse}{LMMSE}{linear minimum mean square error}
\newacronym{ris}{RIS}{reconfigurable intelligent surface}
\newacronym{svd}{SVD}{singular values decomposition}
%	\newacronym{CDF}{cumulative distribution function}
%	\newacronym{PDF}{probability density function}
%	\newacronym{iid}{i.i.d.\@}{independent and identically distributed}
%	\newacronym{iff}{if and only if}

